Attention-based Multi-Reference Learning for Image Super-Resolution

This paper proposes a novel Attention-based Multi-Reference Super-resolution network (AMRSR) that, given a low-resolution image, learns to adaptively transfer the most similar texture from multiple reference images to the super-resolution output whilst maintaining spatial coherence. The use of multiple reference images together with attention-based sampling is demonstrated to achieve significantly improved performance over state-of-the-art reference super-resolution approaches on multiple benchmark datasets. Reference super-resolution approaches have recently been proposed to overcome the ill-posed problem of image super-resolution by providing additional information from a high-resolution reference image. Multi-reference super-resolution extends this approach by providing a more diverse pool of image features to overcome the inherent information deficit whilst maintaining memory efficiency. A novel hierarchical attention-based sampling approach is introduced to learn the similarity between low-resolution image features and multiple reference images based on a perceptual loss. Ablation demonstrates the contribution of both multi-reference and hierarchical attention-based sampling to overall performance. Perceptual and quantitative ground-truth evaluation demonstrates significant improvement in performance even when the reference images deviate significantly from the target image. The project website can be found at https://marcopesavento.github.io/AMRSR/

==> amrsr_arxive/image_files/comparison_short.tex <==

\begin{tabular}{cccc}
            Ground Truth & RCAN~\cite{zhang2018image} & CSNLN~\cite{mei2020image} & RSRGAN~\cite{zhang2019ranksrgan}\\
            \midrule
            References & TTSR~\cite{yang2020learning} & SRNTT~\cite{ZhangSRNTT2019} & AMRSR (ours)\\
            
            %  \includegraphics[width=4in]{amrsr_arxive/images/paper/121_gtf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/121_rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/121_csnln.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/121_rsrganf.png} \\
            %   \includegraphics[width=4in]{amrsr_arxive/images/paper/0121ref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/121_ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/121_srnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/tigeramr.png} \\

             \includegraphics[width=4in]{amrsr_arxive/images/paper/018_gtf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/018_rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/femcsnln.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/018_rsrganf.png} \\
             \includegraphics[width=4in]{amrsr_arxive/images/paper/018ref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/018_ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/018_srnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/018_amrf.png} \\
             \midrule 
            % \includegraphics[width=4in]{amrsr_arxive/images/paper/011_gtf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/011_rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/011_csnlnf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/chiesasrsgan.png} \\
          
            %   \includegraphics[width=4in]{amrsr_arxive/images/paper/011ref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/011_ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/011_srnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/011_amrf.png} \\
             \includegraphics[width=4in]{amrsr_arxive/images/paper/015_gtf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/015_rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/vencsnln.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/015_rsrganf.png} \\
          
             \includegraphics[width=4in]{amrsr_arxive/images/paper/015ref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/015_ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/015_srnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/venamrf.png} \\
             \midrule
             \includegraphics[width=4in]{amrsr_arxive/images/paper/Fountain_s12gtff.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/Fountain_s12rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/Fountain_s12csnlnf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/fountains12srganf.png} \\
             \includegraphics[width=4in]{amrsr_arxive/images/paper/fountainref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/Fountain_s12ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/Fountainsrnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/fountainamrf.png} \\
            \midrule
             \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16gtf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16rcanf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16csnlnf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16srsganf.png} \\
             \includegraphics[width=4in]{amrsr_arxive/images/paper/000002ref.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16ttsrf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16srnttf.png} & \includegraphics[width=4in]{amrsr_arxive/images/paper/000002_s16amrf.png} \\
             
        \end{tabular}


==> amrsr_arxive/image_files/intro.tex <==
\begin{tabular}{cccccccc}

             \includegraphics[width=2in]{amrsr_arxive/images/paper/036ref.png} & \includegraphics[width=2in]{amrsr_arxive/images/paper/036_0mod.png} & \includegraphics[width=2in]{amrsr_arxive/images/paper/036_gt.png} & \includegraphics[width=2in]{amrsr_arxive/images/paper/036_LR.png} & \includegraphics[width=2in]{amrsr_arxive/images/paper/036_csl.png} & \includegraphics[width=2in]{amrsr_arxive/images/paper/036_rank.png}& \includegraphics[width=2in]{amrsr_arxive/images/paper/036_srntt.png} &
             \includegraphics[width=2in]{amrsr_arxive/images/paper/036_amr.png} \\ Ref. images & Ground Truth & GT patch & LR patch & CSNLN& RSRGAN&SRNTT&AMRSR(ours) \\
        \end{tabular}

==> amrsr_arxive/image_files/reference.tex <==

%\begin{tabular}{cccc}
%\multirow{2}{*}{Ground Truth} & GT patch   & 1 ref. & 2 ref. \\ \cline{2-4} 
%                              & References & 4 ref. & 8ref.  \\
%                              
%\multirow[t]{2}{*}{\includegraphics[width=3in]{amrsr_arxive/images/paper/01.png}
%}             &     \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57gt.png}       &   \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref1.png}     &    \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref2.png}    \\
%                              &    \includegraphics[width=3in]{amrsr_arxive/images/paper/000555ref.png}        &    \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref4.png}    &    \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref8.png}    \\
%\multirow[t]{2}{*}{\includegraphics[width=3in]{amrsr_arxive/images/paper/037gt.png}}            &      \includegraphics[width=3in]{amrsr_arxive/images/paper/037orig.png}      &   \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref1.png}    &    \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref2.png}    \\
%                              &      \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref.png}      &   \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref4.png}     &       \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref8.png}
%\end{tabular}
%\begin{tabular}{L{3cm}L{3cm}L{3cm}L{3cm}}
\begin{tabular}{cccc}
Ground Truth & \shortstack{GT patch\\Ref. images}   & \shortstack{1 ref.\\4 ref} & \shortstack{2 ref. \\8 ref.}\\
                              
\includegraphics[width=3in]{amrsr_arxive/images/paper/01.png}             &     \shortstack{\includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57gt.png} \\\includegraphics[width=3in]{amrsr_arxive/images/paper/000555ref.png} }      &   \shortstack{\includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref1.png}  \\ \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref4.png}  }  &   \shortstack{ \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref2.png} \\  \includegraphics[width=3in]{amrsr_arxive/images/paper/000555_s57ref8.png}}  \\
                            
\includegraphics[width=3in]{amrsr_arxive/images/paper/037gt.png}          &      \shortstack{\includegraphics[width=3in]{amrsr_arxive/images/paper/037orig.png} \\ \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref.png}}    &   \shortstack{\includegraphics[width=3in]{amrsr_arxive/images/paper/037ref1.png}\\  \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref4.png}}  &    \shortstack{\includegraphics[width=3in]{amrsr_arxive/images/paper/037ref2.png} \\  \includegraphics[width=3in]{amrsr_arxive/images/paper/037ref8.png}} \\
                             
\end{tabular}


==> amrsr_arxive/table/SR1.tex <==
\begin{tabular}{|cccll|ccllc|}
\hline
\multicolumn{5}{|c|}{\textbf{Classic, GAN \& RefSR}}                                                                                                                                                 & \multicolumn{5}{c|}{\textbf{PSNR oriented}}                                                                                                                                                        \\ \hline
\multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{CU4REF}     & \multicolumn{1}{c|}{Sun80}         & \multicolumn{1}{l|}{HUMAP}         & GEMAP                               & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{CU4REF}     & \multicolumn{1}{c|}{Sun80}         & \multicolumn{1}{l|}{HUMAP}         & \multicolumn{1}{l|}{GEMAP}         \\ \cline{2-5} \cline{7-10} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{Methods}} & \multicolumn{4}{c|}{PSNR/SSIM}                                                                                                                     & \multicolumn{1}{c|}{\multirow{-2}{*}{Methods}} & \multicolumn{4}{c|}{PSNR/SSIM}                                                                                                                    \\ \hline
Bicubic                                         &                                    &                                    &                                    &                                     & SRResNet                                       & 26.28/.7823                        & 29.80/.8121                        & 35.71/.9093                        & 46.06/.9785                        \\
Bilinear                                        &                                    &                                    &                                    &                                     & RRDBNet                                        & 26.22/.7828                        & 29.56/.8053                        & 35.77/.9102                        & 46.25/.9790                        \\
Nearest                                         &                                    &                                    &                                    &                                     & EDSR                                           & 25.52/.7652                        & 28.74/.7876                        & 35.36/.9051                        & 45.92/.9784                        \\
SRGAN                                           & 23.63/.6761                        & 25.97/.6570                        & 31.56/.8551                        & 41.68/.9525                         & MDSR                                           & 26.43/.7822                        & 29.96/.8137                        & 35.84/.9107                        & 46.06/.9784                        \\
ESRGAN                                          & 23.69/.6884                        & 26.42/.7005                        & 32.34/.8664                        & 42.78/.9669                         & NHR                                            &                                    &                                    & 33.13/.8981                        & 36.15/.9544                        \\
ESRGAN+                                         &                                    &                                    &                                    &                                     & NLR                                            &                                    &                                    & 33.13/.8941                        & 42.22/.9731                        \\
RSRGAN                                          & 25.49/.7494                        & 29.10/.7873                        & 33.90/.8892                        & 43.44/.9707                         & RCAN                                           & 26.63/.7880                        & 30.07/.8156                        & {\color[HTML]{3531FF} 36.00/.9123} & {\color[HTML]{3531FF} 46.33/.9791} \\
CrossNet                                        &                                    &                                    &                                    &                                     & MAFFSRN                                        & 26.57/.7853                        & 30.05/.8141                        & 35.78/.9101                        & 46.06/.9785                        \\
SRNTT                                           & {\color[HTML]{3531FF} 26.42/.7738} & {\color[HTML]{3531FF} 29.72/.7984} & {\color[HTML]{3531FF} 34.78/.8963} & {\color[HTML]{3531FF} 45.03/.9743*} & CSNLN                                          & 26.94/.7958                        & {\color[HTML]{3531FF} 30.25/.8197} & 34.24/.9042                        & {\color[HTML]{3531FF} 46.11/.9792} \\
TTSR                                            & 25.23/.7512                        & 28.23/.7595                        & 34.22/.8912                        & 35.32/.9566*                        & SRNTTpsnr                                      & {\color[HTML]{3531FF} 27.62/.8201} & 30.16/.8176                        & 35.91/.9120                        & 46.28/.9791*                       \\
AMRSR                                             &                                    &                                    &                                    &                                     & TTSRpsnr                                       & 26.66/.7875                        & 29.97/.8123                        & 35.35/.9083                        & 37.50/.9709*                       \\
                                                &                                    &                                    &                                    &                                     & AMRSRpsnr                                        &                                    &                                    &                                    &                                    \\ \hline
\end{tabular}

==> amrsr_arxive/table/SR2.tex <==
\begin{tabular}{|c|cccc|}
\hline
Methods   & \multicolumn{1}{c|}{\textbf{CU4REF}} & \multicolumn{1}{c|}{\textbf{Sun80}}                    & \multicolumn{1}{c|}{\textbf{GEMAP}} & \multicolumn{1}{c|}{\textbf{HUMAP}}                      \\ \hline
SRResNet~\cite{ledig2017photo}  & 26.28/.7823                          & 29.80/.8121                                            & 35.71/.9093                         & 46.06/.9785                                              \\
RRDBNet~\cite{wang2018esrgan}   & 26.22/.7828                          & 29.56/.8053                                            & 35.77/.9102                         & 46.25/.9790                                              \\
EDSR~\cite{lim2017enhanced}      & 25.52/.7652                          & 28.74/.7876                                            & 35.36/.9051                         & 45.92/.9784                                              \\
MDSR~\cite{lim2017enhanced}      & 26.43/.7822                          & 29.96/.8137                                            & 35.84/.9107                         & 46.06/.9784                                              \\
NHR~\cite{li2019_3dappearance}       &            --                          &    --                                                    & 33.13/.8981                         & 36.15/.9544                                              \\
NLR~\cite{li2019_3dappearance}       &          --                            &     --                                                   & 33.13/.8941                         & 42.22/.9731                                              \\
RCAN~\cite{zhang2018image}      & 26.63/.7880                          & 30.07/.8156                                            & {\color[HTML]{3531FF} 36.00/.9123}  & {\color[HTML]{3531FF} 46.33/\color[HTML]{000000}.9791}                       \\
MAFFSRN~\cite{muqeet2020ultra}   & 26.57/.7853                          & 30.05/.8141                                            & 35.78/.9101                         & 46.06/.9785                                              \\
CSNLN~\cite{mei2020image}     & 26.94/.7958                          & {\color[HTML]{3531FF} 30.25/.8197}                     & 34.24/.9042                         & { 46.11/\color[HTML]{3531FF}.9792}                       \\
SRNTT-\textit{$l_2$} & {\color[HTML]{3531FF} 27.62/.8201}   & 30.16/.8176                                            & 35.91/.9120*                         & 46.28/.9791*                                             \\
TTSR-\textit{$l_2$}  & 27.02/.8001                          & 29.97/.8123                                            & 35.35/.9083*                         & 37.50/.9709*                                             \\
AMRSR-\textit{$l_2$}   & {\color[HTML]{FF0000}\textbf{28.32/.8394 }  }                       &{\color[HTML]{FF0000}\textbf{ 30.95/.8438 } }                                         &                         {\color[HTML]{FF0000}\textbf{ 36.82/.9248 }  }          &                                               {\color[HTML]{FF0000}\textbf{46.86/.9814}   }        \\ \hline
SRGAN~\cite{ledig2017photo}     & 23.63/.6761                          & \multicolumn{1}{c}{25.97/.6570}                        & 31.56/.8551                         & \multicolumn{1}{c|}{41.68/.9525}                         \\
ESRGAN~\cite{wang2018esrgan}    & 23.69/.6884                          & \multicolumn{1}{c}{26.42/.7005}                        & 32.34/.8664                         & \multicolumn{1}{c|}{42.78/.9669}                         \\
%ESRGAN+   &                                      & \multicolumn{1}{c}{}                                   &                            24.92/.6612         &  \multicolumn{1}{c|}{26.40/.8711}                                    \\
RSRGAN~\cite{zhang2019ranksrgan}    & 25.49/.7494                          & \multicolumn{1}{c}{29.10/.7873}                        & 33.90/.8892                         & \multicolumn{1}{c|}{43.44/.9707}                         \\
CrossNet~\cite{zheng2018crossnet}  &                 26.00/.7576                     & \multicolumn{1}{c}{29.16/.7834}                                   &                                32.95/.8741     & \multicolumn{1}{c|}{30.30/.9317}                                    \\
SSEN~\cite{shim2020robust}  &                 22.71/.7169                     & \multicolumn{1}{c}{26.58/.7824}                                   &                                25.86/.8150     & \multicolumn{1}{c|}{35.61/.9446}                                    \\
SRNTT~\cite{ZhangSRNTT2019}     & {\color[HTML]{3531FF} 26.42/.7738}   & \multicolumn{1}{c}{{\color[HTML]{3531FF} 29.72/.7984}} & {\color[HTML]{3531FF} 34.78/.8963*}  & \multicolumn{1}{c|}{{\color[HTML]{3531FF} 45.03/.9743*}} \\
TTSR~\cite{yang2020learning}      & 25.59/.7645                          & \multicolumn{1}{c}{28.23/.7595}                        & 34.22/.8912*                         & \multicolumn{1}{c|}{35.32/.9566*}                        \\
AMRSR       &{\color[HTML]{FF0000} 27.49/.8145  }                        & \multicolumn{1}{c}{{\color[HTML]{FF0000}30.42/.8263} }                       &                \multicolumn{1}{c}{{\color[HTML]{FF0000}35.80/.9122} }                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000}45.56/.9771}}                                    \\ \hline
\end{tabular}

==> amrsr_arxive/table/SR2_new.tex <==
\begin{tabular}{c|c|cccc|}
\cline{2-6}
&
\multicolumn{1}{c}{\textbf{Methods}}   & \multicolumn{1}{c|}{\textbf{CU4REF}} & \multicolumn{1}{c|}{\textbf{Sun80}}                    & \multicolumn{1}{c|}{\textbf{GEMAP}} & \multicolumn{1}{c|}{\textbf{HUMAP}}                      \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{PSNR-oriented}}}}} & SRResNet~\cite{ledig2017photo}  & 26.28/.7823                          & 29.80/.8121                                            & 35.71/.9093                         & 46.06/.9785                                              \\
\multicolumn{1}{|c|}{}                        &
RRDBNet~\cite{wang2018esrgan}   & 26.22/.7828                          & 29.56/.8053                                            & 35.77/.9102                         & 46.25/.9790                                              \\
\multicolumn{1}{|c|}{}                        &
EDSR~\cite{lim2017enhanced}      & 25.52/.7652                          & 28.74/.7876                                            & 35.36/.9051                         & 45.92/.9784                                              \\
\multicolumn{1}{|c|}{}                        &
MDSR~\cite{lim2017enhanced}      & 26.43/.7822                          & 29.96/.8137                                            & 35.84/.9107                         & 46.06/.9784                                              \\
\multicolumn{1}{|c|}{}                        &
NHR~\cite{li2019_3dappearance}       &            --                          &    --                                                    & 33.13/.8981                         & 36.15/.9544                                              \\
\multicolumn{1}{|c|}{}                        &
NLR~\cite{li2019_3dappearance}       &          --                            &     --                                                   & 33.13/.8941                         & 42.22/.9731                                              \\
\multicolumn{1}{|c|}{}                        &
RCAN~\cite{zhang2018image}      & 26.63/.7880                          & 30.07/.8156                                            & {\color[HTML]{3531FF} 36.00/.9123}  & {\color[HTML]{3531FF} 46.33/\color[HTML]{000000}.9791}                       \\
\multicolumn{1}{|c|}{}                        &
MAFFSRN~\cite{muqeet2020ultra}   & 26.57/.7853                          & 30.05/.8141                                            & 35.78/.9101                         & 46.06/.9785                                              \\
\multicolumn{1}{|c|}{}                        &
CSNLN~\cite{mei2020image}     & 26.94/.7958                          & {\color[HTML]{3531FF} 30.25/.8197}                     & 34.24/.9042                         & { 46.11/\color[HTML]{3531FF}.9792}                       \\
\multicolumn{1}{|c|}{}                        &
SRNTT-\textit{$l_2$} & {\color[HTML]{3531FF} 27.62/.8201}   & 30.16/.8176                                            & 35.91/.9120*                         & 46.28/.9791*                                             \\
\multicolumn{1}{|c|}{}                        &
TTSR-\textit{$l_2$}  & 27.02/.8001                          & 29.97/.8123                                            & 35.35/.9083*                         & 37.50/.9709*                                             \\
\multicolumn{1}{|c|}{}                        &
AMRSR-\textit{$l_2$}   & {\color[HTML]{FF0000}\textbf{28.32/.8394 }  }                       &{\color[HTML]{FF0000}\textbf{ 30.95/.8438 } }                                         &                         {\color[HTML]{FF0000}\textbf{ 36.82/.9248 }  }          &                                               {\color[HTML]{FF0000}\textbf{46.86/.9814}   }        \\ \hline
\multicolumn{1}{|c|}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{Visual-Oriented}}}}}                    & 
SRGAN~\cite{ledig2017photo}     & 23.63/.6761                          & \multicolumn{1}{c}{25.97/.6570}                        & 31.56/.8551                         & \multicolumn{1}{c|}{41.68/.9525}                         \\
\multicolumn{1}{|c|}{}                        &
ESRGAN~\cite{wang2018esrgan}    & 23.69/.6884                          & \multicolumn{1}{c}{26.42/.7005}                        & 32.34/.8664                         & \multicolumn{1}{c|}{42.78/.9669}                         \\
\multicolumn{1}{|c|}{}                        &
%ESRGAN+   &                                      & \multicolumn{1}{c}{}                                   &                            24.92/.6612         &  \multicolumn{1}{c|}{26.40/.8711}                                    \\
RSRGAN~\cite{zhang2019ranksrgan}    & 25.49/.7494                          & \multicolumn{1}{c}{29.10/.7873}                        & 33.90/.8892                         & \multicolumn{1}{c|}{43.44/.9707}                         \\
\multicolumn{1}{|c|}{}                        &
CrossNet~\cite{zheng2018crossnet}  &                 26.00/.7576                     & \multicolumn{1}{c}{29.16/.7834}                                   &                                32.95/.8741     & \multicolumn{1}{c|}{30.30/.9317}                                    \\
\multicolumn{1}{|c|}{}                        &
SSEN~\cite{shim2020robust}  &                 22.71/.7169                     & \multicolumn{1}{c}{26.58/.7824}                                   &                                25.86/.8150     & \multicolumn{1}{c|}{35.61/.9446}                                    \\
\multicolumn{1}{|c|}{}                        &
SRNTT~\cite{ZhangSRNTT2019}     & {\color[HTML]{3531FF} 26.42/.7738}   & \multicolumn{1}{c}{{\color[HTML]{3531FF} 29.72/.7984}} & {\color[HTML]{3531FF} 34.78/.8963*}  & \multicolumn{1}{c|}{{\color[HTML]{3531FF} 45.03/.9743*}} \\
\multicolumn{1}{|c|}{}                        &
TTSR~\cite{yang2020learning}      & 25.59/.7645                          & \multicolumn{1}{c}{28.23/.7595}                        & 34.22/.8912*                         & \multicolumn{1}{c|}{35.32/.9566*}                        \\
\multicolumn{1}{|c|}{}                        &
AMRSR       &{\color[HTML]{FF0000} 27.49/.8145  }                        & \multicolumn{1}{c}{{\color[HTML]{FF0000}30.42/.8263} }                       &                \multicolumn{1}{c}{{\color[HTML]{FF0000}35.80/.9122} }                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000}45.56/.9771}}                                    \\ \hline
\end{tabular}

==> amrsr_arxive/table/SR2_red.tex <==
\begin{tabular}{|c|cccc|}
\hline
Methods   & \multicolumn{1}{c|}{\textbf{CU4REF}} & \multicolumn{1}{c|}{\textbf{Sun80}}                    & \multicolumn{1}{c|}{\textbf{GEMAP}} & \multicolumn{1}{c|}{\textbf{HUMAP}}                      \\ \hline
SRResNet~\cite{ledig2017photo}  & 26.28/.7823                          & 29.80/.8121                                            & 35.71/.9093                         & 46.06/.9785                                              \\
% RRDBNet~\cite{wang2018esrgan}   & 26.22/.7828                          & 29.56/.8053                                            & 35.77/.9102                         & 46.25/.9790                                              \\
% EDSR~\cite{lim2017enhanced}      & 25.52/.7652                          & 28.74/.7876                                            & 35.36/.9051                         & 45.92/.9784                                              \\
MDSR~\cite{lim2017enhanced}      & 26.43/.7822                          & 29.96/.8137                                            & 35.84/.9107                         & 46.06/.9784                                              \\
NHR~\cite{li2019_3dappearance}       &            --                          &    --                                                    & 33.13/.8981                         & 36.15/.9544                                              \\
NLR~\cite{li2019_3dappearance}       &          --                            &     --                                                   & 33.13/.8941                         & 42.22/.9731                                              \\
RCAN~\cite{zhang2018image}      & 26.63/.7880                          & 30.07/.8156                                            & {\color[HTML]{3531FF} 36.00/.9123}  & {\color[HTML]{3531FF} 46.33/\color[HTML]{000000}.9791}                       \\
MAFFSRN~\cite{muqeet2020ultra}   & 26.57/.7853                          & 30.05/.8141                                            & 35.78/.9101                         & 46.06/.9785                                              \\
CSNLN~\cite{mei2020image}     & 26.94/.7958                          & {\color[HTML]{3531FF} 30.25/.8197}                     & 34.24/.9042                         & { 46.11/\color[HTML]{3531FF}.9792}                       \\
SRNTT-\textit{$l_2$} & {\color[HTML]{3531FF} 27.62/.8201}   & 30.16/.8176                                            & 35.91/.9120*                         & 46.28/.9791*                                             \\
TTSR-\textit{$l_2$}  & 27.02/.8001                          & 29.97/.8123                                            & 35.35/.9083*                         & 37.50/.9709*                                             \\
AMRSR-\textit{$l_2$}   & {\color[HTML]{FF0000}\textbf{28.32/.8394 }  }                       &{\color[HTML]{FF0000}\textbf{ 30.95/.8438 } }                                         &                         {\color[HTML]{FF0000}\textbf{ 36.82/.9248 }  }          &                                               {\color[HTML]{FF0000}\textbf{46.86/.9814}   }        \\ \hline
SRGAN~\cite{ledig2017photo}     & 23.63/.6761                          & \multicolumn{1}{c}{25.97/.6570}                        & 31.56/.8551                         & \multicolumn{1}{c|}{41.68/.9525}                         \\
ESRGAN~\cite{wang2018esrgan}    & 23.69/.6884                          & \multicolumn{1}{c}{26.42/.7005}                        & 32.34/.8664                         & \multicolumn{1}{c|}{42.78/.9669}                         \\
%ESRGAN+   &                                      & \multicolumn{1}{c}{}                                   &                            24.92/.6612         &  \multicolumn{1}{c|}{26.40/.8711}                                    \\
RSRGAN~\cite{zhang2019ranksrgan}    & 25.49/.7494                          & \multicolumn{1}{c}{29.10/.7873}                        & 33.90/.8892                         & \multicolumn{1}{c|}{43.44/.9707}                         \\
CrossNet~\cite{zheng2018crossnet}  &                 26.00/.7576                     & \multicolumn{1}{c}{29.16/.7834}                                   &                                32.95/.8741     & \multicolumn{1}{c|}{30.30/.9317}                                    \\
SSEN~\cite{shim2020robust}  &                 22.71/.7169                     & \multicolumn{1}{c}{26.58/.7824}                                   &                                25.86/.8150     & \multicolumn{1}{c|}{35.61/.9446}                                    \\
SRNTT~\cite{ZhangSRNTT2019}     & {\color[HTML]{3531FF} 26.42/.7738}   & \multicolumn{1}{c}{{\color[HTML]{3531FF} 29.72/.7984}} & {\color[HTML]{3531FF} 34.78/.8963*}  & \multicolumn{1}{c|}{{\color[HTML]{3531FF} 45.03/.9743*}} \\
TTSR~\cite{yang2020learning}      & 25.59/.7645                          & \multicolumn{1}{c}{28.23/.7595}                        & 34.22/.8912*                         & \multicolumn{1}{c|}{35.32/.9566*}                        \\
AMRSR       &{\color[HTML]{FF0000} 27.49/.8145  }                        & \multicolumn{1}{c}{{\color[HTML]{FF0000}30.42/.8263} }                       &                \multicolumn{1}{c}{{\color[HTML]{FF0000}35.80/.9122} }                      & \multicolumn{1}{c|}{{\color[HTML]{FF0000}45.56/.9771}}                                    \\ \hline
\end{tabular}

==> amrsr_arxive/table/allconfig.tex <==
\begin{tabular}{|c|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Configurations}} & \multicolumn{4}{c|}{\textit{\textbf{Visual-Oriented}}}                                                       & \multicolumn{4}{c|}{\textit{\textbf{PSNR-Oriented}}}                                                         \\ \cline{2-9} 
                                         & \multicolumn{1}{c|}{CU4REF} & \multicolumn{1}{c|}{Sun80} & \multicolumn{1}{c|}{GEMAP} & HUMAP                & \multicolumn{1}{c|}{CU4REF} & \multicolumn{1}{c|}{Sun80} & \multicolumn{1}{c|}{GEMAP} & HUMAP                \\ \hline
$N_{I}=1,N_{R}=1$                       & \textbf{27.49/.8145}                 & 30.14/.8170                & 35.58/.9077                & 45.55/.9771          & \textbf{28.32/.8394}                 & 30.84/.8393                & 36.60/.9221                & 46.81/.9811          \\
$N_{I}=1,N_{R}=4$                       & 27.17/.8073                 & 30.30/.8217                & 35.63/.9106                & 45.45/.9762 & 28.00/.8358                 & 30.87/.8415                & 36.65/.9232                & 46.85/.9814          \\
$N_{I}=1,N_{R}=16$                      & 27.08/.8040                 & \textbf{30.42/.8263}                & \textbf{35.80/.9122}       & \textbf{45.56/.9771}          & 27.97/.8341                 & \textbf{30.95/.8438}       & \textbf{36.82/.9248}                & \textbf{46.86/.9814} \\
$N_{I}=4,N_{R}=1$                       & 26.44/.7793                 & 29.86/.8082                & 35.49/.9059                & 45.39/.9761          & 27.28/.8108                 & 30.62/.8329                & 36.57/.9219                & 46.81/.9812          \\
$N_{I}=4,N_{R}=4$                       & 26.43/.7776                 & 30.04/.8131                & 35.50/.9071                & 45.34/.9754          & 27.22/.8096                 & 30.61/.8332                & 36.59/.9225                & 46.82/.9812          \\
$N_{I}=4,N_{R}=16$                      & 26.38/.7749                 & 30.17/.8167                & 35.65/.9111                & 45.38/.9762          & 27.16/.8068                 & 30.69/.8360                & 36.69/.9236                & 46.80/.9811          \\
$N_{I}=16,N_{R}=1$                      & 25.58/.7405                 & 29.76/.8024                & 35.42/.9055                & 45.40/.9760          & 26.45/.7809                 & 30.51/.8292                & 36.53/.9215                & 46.81/.9810          \\
$N_{I}=16,N_{R}=4$                      & 25.63/.7441                 & 29.89/.8075                & 35.46/.9061                & 45.24/.9753          & 26.40/.7830                 & 30.48/.8284                & 36.54/.9217                & 46.74/.9808          \\
$N_{I}=16,N_{R}=16$                     & 25.62/.7415                 & 29.90/.8082                & 35.57/.9101                & 45.33/.9760          & 26.36/.7789                 & 30.47/.8299                & 36.60/.9229                & 46.74/.9808          \\ \hline
\end{tabular}

==> amrsr_arxive/table/allmemory.tex <==
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Configurations}} & \multicolumn{2}{c|}{\textbf{CU4REF}}                                    & \multicolumn{2}{c|}{\textbf{Sun80}}                                     & \multicolumn{2}{c|}{\textbf{GEMAP}}                                     & \multicolumn{2}{c|}{\textbf{HUMAP}}                                     \\ \cline{2-9} 
                                          & \multicolumn{1}{c|}{GPU} & Time  & \multicolumn{1}{c|}{GPU} & Time & \multicolumn{1}{c|}{GPU} & Time & \multicolumn{1}{c|}{GPU} & Time \\ \hline
$N_{I}=1,N_{R}=1$                                & 1.36                         & \textbf{46.73}                      & 3.96                         & \textbf{80.62}                 & 40.15                        & \textbf{126.91}              & 29.60                        & \textbf{147.26}  \\
$N_{I}=1,N_{R}=4$                                   & 1.21                         & 137.41           & 3.23                         & 154.03                  & 28.49                        & 265.73             & 20.98                        & 161.27  \\
$N_{I}=1,N_{R}=16$                                         & 1.22                         & 270.76                   & 3.24                         & 391.63                  & 15.69                        & 265.14               & 11.59                        & 159.63  \\
$N_{I}=4,N_{R}=1$                                     & 1.00                         & 65.74                  & 3.33                         & 112.81             & 39.54                        & 240.00                    & 26.93                        & 275.27  \\
$N_{I}=4,N_{R}=4$                                   & 0.80                         & 77.46                   & 2.06                         & 155.39                    & 28.18                        & 545.41                   & 20.73                        & 310.19  \\
$N_{I}=4,N_{R}=16$                                   & 0.80                         & 168.98                & 2.08                         & 372.73                   & 15.53                        & 483.30                  & 11.44                        & 430.83  \\
$N_{I}=16,N_{R}=1$                              & 0.90                         & 56.19                   & 3.17                         & 129.62                      & 39.29                        & 252.81                     & 26.77                        & 380.07  \\
$N_{I}=16,N_{R}=4$                                    & \textbf{0.72}                         & 76.85                & \textbf{1.79}                         & 204.95            & 28.06                        & 1072.46              & 20.63                        & 635.21  \\
$N_{I}=16,N_{R}=16$                              & 0.73                         & 168.70              & 1.80                         & 470.91              & \textbf{15.47}                        & 968.72            & \textbf{11.39}                        & 716.55  \\ \hline
\end{tabular}

==> amrsr_arxive/table/arch.tex <==
\begin{tabular}{|c|c|}
\hline
\textbf{Id}    & \textbf{Network Layers}                    \\ \hline
0 & ImgFeature=Residual Blocks(Input) \\\hline
1  &   Concat: ImgFeature, $O_3$                    \\ \hline
2  & Conv, LeakyReLU   \\ \hline
3-18    & Residual Blocks (Conv,ReLu,Conv)               \\ \hline
19     & ImgFeature + output18                  \\ \hline
20  & Conv, PixelShuffle(2x), LeakyReLU   \\ \hline
21   & Concat:output20,$O_2$               \\ \hline
22    & Conv, LeakyReLU \\ \hline
23-30    & Residual Blocks (Conv,ReLu,Conv)           \\ \hline
31   & output20+output30                   \\ \hline
32 & Conv, PixelShuffle(2x), LeakyReLU   \\ \hline
33    & Concat:output32,$O_1$               \\ \hline
34    & Conv, LeakyReLU \\ \hline
35-38    & Residual Blocks (Conv,ReLu,Conv)           \\ \hline
39    & output32+output38                   \\ \hline
40 & Conv, PixelShuffle(2x), LeakyReLU   \\ \hline
\end{tabular}

==> amrsr_arxive/table/attention.tex <==
\begin{tabular}{|c|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Config.}} & \multicolumn{4}{c|}{\textit{\textbf{Visual-Oriented}}}                                                          & \multicolumn{4}{c|}{\textit{\textbf{PSNR-Oriented}}}                                                            \\ \cline{2-9} 
                                  & \multicolumn{1}{c}{CU4REF} & \multicolumn{1}{c}{Sun80} & \multicolumn{1}{c}{GEMAP} & \multicolumn{1}{c|}{HUMAP} & \multicolumn{1}{c}{CU4REF} & \multicolumn{1}{c}{Sun80} & \multicolumn{1}{c}{GEMAP} & \multicolumn{1}{c|}{HUMAP} \\ \hline
No attention                      & 27.05/.8026                & 29.72/.7997               & 35.02/.9003               & 45.25/.9746                & 27.54/.8170                & 30.18/.8171            & 35.91/.9130               & 46.33/.9791                \\
Ref. attention                    & 26.78/.7909                &             29.84/.8022              & 35.11/.9003               & 45.28/.9753                & 27.55/.8179                &             30.21/.8196              & 35.93/.9131               & 46.43/.9794                \\
Both attention                    & 26.52/.7795                & 29.73/.7982               & 35.16/.9015               & 45.35/.9754                & 27.18/.8064                & 30.24/.8194               & 35.91/.9130               & 46.43/.9793                \\
AMRSR                               & \textbf{27.49/.8145       }         & \textbf{30.41/.8257 }              &                     \textbf{35.80/.9122}      & \textbf{45.56/.9771}       & \textbf{28.32/.8394 }               & \textbf{30.95/.8438   }            &          \textbf{36.82/.9248}                 & \textbf{46.86/.9814}       \\ \hline
\end{tabular}

==> amrsr_arxive/table/attention_psnr.tex <==
\begin{tabular}{|c|cccc|}
\hline
\textbf{Config.} &\textbf{CU4REF} & \textbf{Sun80} & \textbf{GEMAP} & \textbf{HUMAP} \\ \hline
No attention                                     & 27.54/.8170                & 30.18/.8171            & 35.91/.9130               & 46.33/.9791                \\
Ref. attention                                  & 27.55/.8179                &             30.21/.8196              & 35.93/.9131               & 46.43/.9794                \\
Both attention                                    & 27.18/.8064                & 30.24/.8194               & 35.91/.9130               & 46.43/.9793                \\
AMRSR                                 & \textbf{28.32/.8394 }               & \textbf{30.95/.8438   }            &          \textbf{36.82/.9248}                 & \textbf{46.86/.9814}       \\ \hline
\end{tabular}

==> amrsr_arxive/table/attention_visual.tex <==
\begin{tabular}{c|c|cccc|}
\cline{2-6}
&
\textbf{Config.} &\textbf{CU4REF} & \textbf{Sun80} & \textbf{GEMAP} & \textbf{HUMAP} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{\scriptsize	 Visual-Oriented}}}}} &
No attention                                    & 27.05/.8026                & 29.72/.7997               & 35.02/.9003               & 45.25/.9746                 \\
\multicolumn{1}{|c|}{}  &
Ref. attention                                 & 26.78/.7909                &             29.84/.8022              & 35.11/.9003               & 45.28/.9753                \\
\multicolumn{1}{|c|}{}  &
Both attention                                     & 26.52/.7795                & 29.73/.7982               & 35.16/.9015               & 45.35/.9754                 \\
\multicolumn{1}{|c|}{}  &
AMRSR                                  & \textbf{27.49/.8145       }         & \textbf{30.41/.8257 }              &                     \textbf{35.80/.9122}      & \textbf{45.56/.9771}        \\ \hline
\end{tabular}

==> amrsr_arxive/table/cimr.tex <==
\begin{tabular}{|c|cccc|}
\hline
\multicolumn{1}{|c|}{\textbf{Algorithms}} & \multicolumn{1}{c|}{\bf L1} & \multicolumn{1}{c|}{\bf L2} & \multicolumn{1}{c|}{\bf L3} & \bf L4         \\ \hline
CIMR-\textit{$l_2$}                         & 27.32/.805              & 27.05/.799              & 26.92/.796              & 26.86/.794 \\
AMRSR-\textit{$l_2$}                          & \textbf{28.38/.844}              & \textbf{27.87/.825}     & \textbf{27.76/.821}              & \textbf{27.59/.817} \\ \hline
CIMR~\cite{cui2020towards}                             & 26.50/.786              & 26.47/.784              & 26.45/.784              & 26.44/.784 \\
AMRSR                              & 27.32/.808              & 27.01/.795              & 26.95/.793              & 26.85/.791 \\ \hline
\end{tabular}

==> amrsr_arxive/table/memory.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{3}{c|}{\textbf{CU4REF}}                                    & \multicolumn{3}{c|}{\textbf{Sun80}}                                     & \multicolumn{3}{c|}{\textbf{GEMAP}}                                     & \multicolumn{3}{c|}{\textbf{HUMAP}}                                     \\ \cline{2-13} 
                                  & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{GPU(GB)} & Time(s) & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{GPU(GB)} & Time(s) & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{GPU(GB)} & Time(s) & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{GPU(GB)} & Time(s) \\ \hline
AMRSR 1ref                          & 27.92/.8293                    & 1.01                         & 20.03   & 30.61/.8376                    & 2.10                         & 113.36  &              36.49/.9219                 & 15.57                        & 84.28   &        46.64/.9803                        & 11.47                        & 44.05   \\
AMRSR 2ref                          & 28.26/.8384                    & 1.25                         & 41.78   & 30.79/.8380                    & 2.66                         & 204.38  & 36.56/.9228                    & 15.63                      & 104.85  & 46.74/.9808                    & 11.53                     & 84.24   \\
AMRSR 8ref                          & --                             & --                           & --      & --                             & --                           & --      & 36.84/.9255                    & 15.80                        & 418.82  &                46.87/.9814                & 11.70                        & 316.04  \\
$N_{R}=1$                        & 28.32/.8394                    & 1.36                         & 46.73   & 30.84/.8393                    & 3.96                         & 80.62   &            36.60/.9221                     & 40.15                        & 126.91  &              46.81/.9811                  & 29.60                        & 147.26  \\
$N_{R}=4$                        & 28.00/.8358                    & 1.21                         & 137.41  & 30.87/.8415                    & 3.23                         & 154.03  & 36.65/.9232                   & 28.49                        & 265.73  & 46.85/.9814                    & 20.98                        & 161.27  \\
$N_{R}=16$                       & 27.97/.8341                    & 1.22                         & 270.76  & 30.95/.8438                    & 3.24                         & 391.63  &             36.82/.9248                   & 15.69                        & 265.14  & 46.86/.9814                    & 11.59                        & 159.63  \\
cut 1ref                       & --                             & --                           & --      & --                             & --                           & --      &              36.44/.9205              & 3.99                         & 23.13   &                46.63/ .9802                & 2.94                         & 20.31   \\
cut 4ref                       & --                             & --                           & --      & --                             & --                           & --      &                 36.75/.9242               & 4.10                         & 111.65  & 46.81/.9811                    & 3.06                         & 98.95   \\
SRNTT~\cite{ZhangSRNTT2019}                             & 27.62/.8201                    & 2.81                         & 20.87   & 30.16/.8176                    & 14.63                        & 26.93   & 35.91/.9120                    & $>$ 48(26.51)                & (10.37) & 46.28/.9791                    & $>$ 48(19.49)                & (15.37) \\
TTSR~\cite{yang2020learning}                              & 27.02/.8001                    & 4.24                         & 17.03   & 29.97/.8123                    & 20.61                        & 17.60   & 35.35/.9083                    & $>$ 48(40.07)                & (17.13) & 37.50/.9709                    & $>$ 48(29.47)                & (10.31) \\ \hline
\end{tabular}

==> amrsr_arxive/table/memory2.tex <==
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{2}{c|}{\textbf{CU4REF}}                                    & \multicolumn{2}{c|}{\textbf{Sun80}}                                     & \multicolumn{2}{c|}{\textbf{GEMAP}}                                     & \multicolumn{2}{c|}{\textbf{HUMAP}}                                     \\ \cline{2-9} 
                                  & PSNR/SSIM & GPU &  PSNR/SSIM & GPU &  PSNR/SSIM & GPU & PSNR/SSIM & GPU  \\ \hline
AMRSR 1                          & 27.92/.8293                    & 1.01                          & 30.61/.8376                    & 2.10                         &              36.49/.9219                 & 15.57                          &        46.64/.9803                        & 11.47                          \\
AMRSR 2                          & 28.26/.8384                    & 1.25                       & 30.79/.8380                    & 2.66                          & 36.56/.9228                    & 15.63                     & 46.74/.9808                    & 11.53                      \\
AMRSR 8                         & --                             & --                                 & --                             & --                              & 36.84/.9255                    & 15.80                        &                46.87/.9814                & 11.70                    \\
$N_{R}=1$                        & 28.32/.8394                    & 1.36                         & 30.84/.8393                    & 3.96                         &            36.60/.9221                     & 40.15                    &              46.81/.9811                  & 29.60                        \\
$N_{R}=4$                        & 28.00/.8358                    & 1.21                        & 30.87/.8415                    & 3.23                      & 36.65/.9232                   & 28.49                     & 46.85/.9814                    & 20.98                      \\
$N_{R}=16$                       & 27.97/.8341                    & 1.22                        & 30.95/.8438                    & 3.24                        &             36.82/.9248                   & 15.69              & 46.86/.9814                    & 11.59                         \\
cut 1                      & --                             & --                               & --                             & --                              &              36.44/.9205              & 3.99                       &                46.63/.9802                & 2.94              \\
cut 4                      & --                             & --                             & --                             & --                              &                 36.75/.9242               & 4.10                         & 46.81/.9811                    & 3.06                       \\
SRNTT~\cite{ZhangSRNTT2019}                             & 27.62/.8201                    & 2.81                           & 30.16/.8176                    & 14.63                         & 35.91/.9120                    & (26.51)              & 46.28/.9791                    & (19.49)                \\
TTSR~\cite{yang2020learning}                              & 27.02/.8001                    & 4.24                        & 29.97/.8123                    & 20.61                    & 35.35/.9083                    &  (40.07)                 & 37.50/.9709                    & (29.47)               \\ \hline
\end{tabular}

==> amrsr_arxive/table/memory3.tex <==
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{2}{c|}{\textbf{CU4REF}}                                    & \multicolumn{2}{c|}{\textbf{Sun80}}                                     & \multicolumn{2}{c|}{\textbf{GEMAP}}                                     & \multicolumn{2}{c|}{\textbf{HUMAP}}                                     \\ \cline{2-9} 
                                  & \footnotesize{PSNR/SSIM} & \footnotesize{GPU} &  \footnotesize{PSNR/SSIM} & \footnotesize{GPU} &  \footnotesize{PSNR/SSIM} & \footnotesize{GPU} & \footnotesize{PSNR/SSIM} & \footnotesize{GPU}  \\ \hline
AMRSR 1                          & 27.92/.829                   & \textbf{1.01}                          & 30.61/.837                 & \textbf{2.10}                         &              36.49/.921           & 15.57                          &        46.64/.980               & 11.47                          \\
AMRSR 2                          & 28.26/.838                   & 1.25                       & 30.79/.838            & 2.66                          & 36.56/.922           & 15.63                     & 46.74/.980                 & 11.53                      \\
AMRSR 8                         & --                             & --                                 & --                             & --                              & \textbf{36.84/.925}                    & 15.80                        &               \textbf{46.87/.981}               & 11.70                    \\
$N_{R}=1$                        & \textbf{28.32/.839}                    & 1.36                         & 30.84/.839               & 3.96                         &            36.60/.922                & 40.15                    &              46.81/.981                 & 29.60                        \\
$N_{R}=4$                        & 28.00/.835                    & 1.21                        & 30.87/.841                    & 3.23                      & 36.65/.923                   & 28.49                     & 46.85/.981                    & 20.98                      \\
$N_{R}=16$                       & 27.97/.834                    & 1.22                        & \textbf{30.95/.843}                    & 3.24                        &             36.82/.924                   & 15.69              & 46.86/.981                    & 11.59                         \\
cut 1                      & --                             & --                               & --                             & --                              &              36.44/.920              & \textbf{3.99}                       &                46.63/.980                & \textbf{2.94}              \\
cut 4                      & --                             & --                             & --                             & --                              &                 36.75/.924               & 4.10                         & 46.81/.981                    & 3.06                       \\
SRNTT~\cite{ZhangSRNTT2019}                             & 27.62/.820                    & 2.81                           & 30.16/.817                   & 14.63                         & 35.91/.912                    & (26.51)              & 46.28/.979                    & (19.49)                \\
TTSR~\cite{yang2020learning}                              & 27.02/.800                    & 4.24                        & 29.97/.812                    & 20.61                    & 35.35/.908                    &  (40.07)                 & 37.50/.970                   & (29.47)               \\ \hline
\end{tabular}

==> amrsr_arxive/table/reference_visual.tex <==
\begin{tabular}{c|c|cccc|}
\cline{2-6}
&
\textbf{Nr. references} & \textbf{CU4REF} & \textbf{Sun80} & \textbf{GEMAP} & \textbf{HUMAP} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{\textit{\small Visual-Oriented}}}}} &
1 Reference                                         & 26.77/.7882                        & 30.15/.8162                        &          35.64/.9106                 &     45.38/.9760                  \\
\multicolumn{1}{|c|}{}  &
2 References                                          & 27.30/.8087                       & 30.27/.8205                        & 35.65/.9108               & 45.45/.9763               \\
\multicolumn{1}{|c|}{}  &
4 References                           & \textbf{27.49/.8145 }                      &  \textbf{30.41/.8257}                        &      35.80/.9122                     &\textbf{ 45.56/.9771    }            \\
\multicolumn{1}{|c|}{}  &
8 References                          & --                                 & --                                 &     \textbf{35.87/.9145}        &         45.50/.9767                     \\

\cline{2-6}
\multicolumn{1}{|c|}{}  &
$2^{nd}$ best                               & 26.42/.7738 & 29.72/.7984 & 34.78/.8963               & 45.03/.9743                \\ \hline
\end{tabular}

==> amrsr_arxive/table/references.tex <==
\begin{tabular}{|c|cccc|cccc|}
\hline
                                          & \multicolumn{4}{c|}{\textit{\textbf{Visual-Oriented}}}                                                                           & \multicolumn{4}{c|}{\textit{\textbf{PSNR-Oriented}}}                                                            \\ \cline{2-9} 
\multirow{-2}{*}{\textbf{Nr. references}} & \multicolumn{1}{c}{CU4REF}         & \multicolumn{1}{c}{Sun80}          & \multicolumn{1}{c}{GEMAP} & \multicolumn{1}{c|}{HUMAP} & \multicolumn{1}{c}{CU4REF} & \multicolumn{1}{c}{Sun80} & \multicolumn{1}{c}{GEMAP} & \multicolumn{1}{c|}{HUMAP} \\ \hline
1 Reference                               & 26.77/.7882                        & 30.15/.8162                        &          35.64/.9106                 &     45.38/.9760                      & 27.92/.8293                & 30.61/.8376               &              36.49/.9219             &                    46.64/.9803        \\
2 References                              & 27.30/.8087                       & 30.27/.8205                        & 35.65/.9108               & 45.45/.9763                & 28.26/.8398                & 30.79/.8380               & 36.58/.9230              & 46.74/.9808                \\
4 References                              & \textbf{27.49/.8145 }                      &  \textbf{30.41/.8257}                        &      35.80/.9122                     &\textbf{ 45.56/.9771    }            & \textbf{28.32/.8394 }               & \textbf{30.95/.8438}             &         36.82/.9248               & 46.86/.9814                \\
8 References                              & --                                 & --                                 &     \textbf{35.87/.9145}        &         45.50/.9767                   & --                         & --                        & \textbf{36.84/.9255 }              &             \textbf{46.87/.9814 }              \\ \hline
$2^{nd}$ best                             & 26.42/.7738 & 29.72/.7984 & 34.78/.8963               & 45.03/.9743                & 27.62/.8201                & 30.25/.8197               & 36.00/.9123               & 46.33/.9792                \\ \hline
\end{tabular}

==> amrsr_arxive/table/references_psnr.tex <==
\begin{tabular}{|c|cccc|}
\hline
\textbf{Nr. references} & \textbf{CU4REF} & \textbf{Sun80} & \textbf{GEMAP} & \textbf{HUMAP} \\ \hline
1 Reference                                          & 27.92/.8293                & 30.61/.8376               &              36.49/.9219             &                    46.64/.9803        \\
2 References                                          & 28.26/.8384                & 30.79/.8380               & 36.58/.9230              & 46.74/.9808                \\
4 References                               & \textbf{28.32/.8394 }               & \textbf{30.95/.8438}             &         36.82/.9248               & 46.86/.9814                \\
8 References                                             & --                         & --                        & \textbf{36.84/.9255 }              &             \textbf{46.87/.9814 }              \\ \hline
$2^{nd}$ best                                 & 27.62/.8201                & 30.25/.8197               & 36.00/.9123               & 46.33/.9792                \\ \hline
\end{tabular}

==> amrsr_arxive/table/sim.tex <==
\begin{tabular}{|c|ccccccc|}
\hline
       & \multicolumn{1}{c|}{TTSR~\cite{yang2020learning}} & \multicolumn{1}{c|}{SRNTT~\cite{ZhangSRNTT2019}} & \multicolumn{1}{c|}{CrossNet~\cite{zheng2018crossnet}} & \multicolumn{1}{c|}{SSEN~\cite{shim2020robust}} & \multicolumn{1}{c|}{AMRSR 1ref} & \multicolumn{1}{c|}{AMRSR 2ref} & AMRSR         \\ \hline
Visual & 25.08/.7468               & 26.17/.7654                & 25.98/.7582                   & 22.83/.7148               & 26.36/.7750                   & 26.43/.7789                   & \textbf{26.47/.7807} \\
PSNR   & 26.59/.7849               & 26.67/.7903                & --                            & --                        & 27.06/.8051                   & 27.09/.8057                   & \textbf{27.10/.8060} \\ \hline
\end{tabular}

==> amrsr_arxive/table/sim2.tex <==
\begin{tabular}{|c|cccccc|}
\hline
       & \multicolumn{1}{c|}{TTSR~\cite{yang2020learning}} & \multicolumn{1}{c|}{SRNTT~\cite{ZhangSRNTT2019}} & \multicolumn{1}{c|}{CrossNet~\cite{zheng2018crossnet}} & \multicolumn{1}{c|}{SSEN~\cite{shim2020robust}} & \multicolumn{1}{c|}{AMRSR 1} & AMRSR         \\ \hline
Visual & 25.08/.746               & 26.17/.765              & 25.98/.758                   & 22.83/.7148               & 26.36/.775                              & \textbf{26.47/.780} \\
PSNR   & 26.59/.784               & 26.67/.790          & --                            & --                        & 27.06/.805                               & \textbf{27.10/.806} \\ \hline
\end{tabular}

==> amrsr_arxive/table/simlevel.tex <==
\begin{tabular}{|c|cccc|}
\hline
\multicolumn{1}{|c|}{\bf Algorithms} & \multicolumn{1}{c|}{\bf L1} & \multicolumn{1}{c|}{\bf L2} & \multicolumn{1}{c|}{\bf L3} & \bf L4                   \\ \hline
Cross-Net~\cite{zheng2018crossnet}                        & 25.98/.7582             & 25.98/.7582             & 25.97/.7581             & 25.97/.7581          \\
SSEN~\cite{shim2020robust}                     & 22.71/.7169             & 22.43/.7114             & 22.30/.7131             & 22.13/.7084          \\
SRNTT~\cite{ZhangSRNTT2019}                           & 26.42/.7738             & 26.34/.7690             & 26.27/.7682             & 26.24/.7678          \\
TTSR~\cite{yang2020learning}                             & 25.59/.7645             & 25.08/.7442             & 24.98/.7414             & 24.95/.7412          \\
AMRSR 1ref                         & 26.77/.7882             & 26.71/.7869             & 26.63/.7841             & 26.48/.7804          \\ \hline
SRNTT-\textit{$l_2$}                       & 27.62/.8201             & 27.21/.8039             & 27.05/.8003             & 26.92/.7969          \\
TTSR-\textit{$l_2$}                         & 27.02/.8001             & 26.48/.7809             & 26.40/.7792             & 26.35/.7784          \\
AMRSR 1-\textit{$l_2$}                        & \textbf{27.92/.8293}    & \textbf{27.51/.8152}    & \textbf{27.40/.8114}    & \textbf{27.24/.8080} \\ \hline
\end{tabular}

==> amrsr_arxive/table/time.tex <==
\begin{tabular}{|c|cccc|}
\hline\
\textbf{Algorithms} & \textbf{CU4REF}                                & \textbf{Sun80}                                    & \textbf{GEMAP}                                 & \textbf{HUMAP}                                
\\ \hline
AMRSR 1ref                         & 20.03                        & 113.36      & 84.28                   & 44.05   \\
AMRSR 2ref                                            & 41.78        & 204.38     & 104.85                & 84.24   \\
AMRSR 8ref                           & --        & --           & 418.82  &               316.04  \\
$N_{R}=1$                                       & 46.73     & 80.62     & 126.91    & 147.26  \\
$N_{R}=4$                                          & 137.41          & 154.03         & 265.73    & 161.27  \\
$N_{R}=16$                                          & 270.76  & 391.63  & 265.14    & 159.63  \\
cut 1ref                                             & --       & --      & 21.95      & 19.08   \\
cut 4ref                                           & --      & --                            & 111.65      & 98.95   \\
SRNTT~\cite{ZhangSRNTT2019}                                 & 20.87     & 26.93             & (19.37)          & (15.37) \\
TTSR~\cite{yang2020learning}                                & \textbf{17.03}       & \textbf{17.60}      & \textbf{(17.13)}          & \textbf{(10.31)} \\ \hline
\end{tabular}

==> amrsr_arxive/table/time_v2.tex <==
\begin{tabular}{|c|cccc|}
\hline\
\textbf{Algorithms} & \textbf{CU4REF}                                & \textbf{Sun80}                                    & \textbf{GEMAP}                                 & \textbf{HUMAP}                                
\\ \hline
AMRSR 1ref                         & 20.03                        & 113.36      & 84.28                   & 44.05   \\
AMRSR 2ref                                            & 41.78        & 204.38     & 104.85                & 84.24   \\
AMRSR 8ref                           & --        & --           & 418.82  &               316.04  \\
$N_{R}=1$                                       & 46.73     & 80.62     & 126.91    & 147.26  \\
$N_{R}=4$                                          & 137.41          & 154.03         & 265.73    & 161.27  \\
$N_{R}=16$                                          & 270.76  & 391.63  & 265.14    & 159.63  \\
cut 1ref                                             & --       & --      & 21.95      & 19.08   \\
cut 4ref                                           & --      & --                            & 111.65      & 98.95   \\
SRNTT~\cite{ZhangSRNTT2019}                                 & 20.87     & 26.93             & (19.37)          & (15.37) \\
TTSR~\cite{yang2020learning}                                & 17.03       & 17.60      & (17.13)         & (10.31)\\
MASA~\cite{lu2021masa}                                & \textbf{5.36}       & \textbf{5.41}      & \textbf{(9.62)}          & \textbf{(7.66)} \\ \hline
\end{tabular}
